Measurement of charm fragmentation ratios and fractions in photoproduction at HERA

The production of D^*+, D^0, D^+, D_s^+ and Lambda_c^+ charm hadrons and their antiparticles in ep scattering at HERA was measured with the ZEUS detector using an integrated luminosity of 79 pb^-1. The measurement has been performed in the photoproduction regime with the exchanged-photon virtuality Q^2 < 1 GeV^2 and for photon-proton centre-of-mass energies in the range 130 < W < 300 GeV. The charm hadrons were reconstructed in the range of transverse momentum p_T(D, Lambda_c) > 3.8 GeV and pseudorapidity |eta(D, Lambda_c)| < 1.6. The production cross sections were used to determine the ratio of neutral and charged D-meson production rates, R_u/d, the strangeness-suppression factor, gamma_s, and the fraction of charged D mesons produced in a vector state, P_v^d. The measured R_u/d and gamma_s values agree with those obtained in deep inelastic scattering and in e^+e^- annihilations. The measured P_v^d value is smaller than, but consistent with, the previous measurements. The fractions of c quarks hadronising as a particular charm hadron, f(c -> D, Lambda_c), were derived in the given kinematic range. The measured open-charm fragmentation fractions are consistent with previous results, although the measured f(c -> D^*+) is smaller and f(c -> Lambda_c^+) is larger than those obtained in e^+e^- annihilations. These results generally support the hypothesis that fragmentation proceeds independently of the hard sub-process.

==> com_def_tex/journal_def.tex <==
% A useful Journal macro
\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

% Some useful journal names
\def\NCA{{\em Nuovo Cimento}}
\def\NIM{{\em Nucl. Instrum. Methods}}
\def\NIMA{{\em Nucl. Instrum. Methods} A}
\def\NPA{{\em Nucl. Phys.} A}
\def\NPB{{\em Nucl. Phys.} B}
\def\PLB{{\em Phys. Lett.}  B}
\def\PR{{\em Phys. Reports} }
\def\PRA{{\em Phys. Reports}  A}
\def\PRL{{\em Phys. Rev. Lett.} }
\def\PRD{{\em Phys. Rev.} D}
\def\ZPC{{\em Z. Phys.} C}
\def\EPC{{\em Eur. Phys. J.} C}
\def\CPC{{\em Comp. Phys. Comm.} }
\def\CNPP{{\em Comm. Nucl. Part. Phys.} }
%
\def\SJNP{{\em Sov. J. Nucl. Phys.} }
\def\CJPB{{\em Czech. J. Phys.} B}
\def\IJMA{{\em Int. J. Mod. Phys.} A}
\def\RMP{{\em Rev. Mod. Phys.} }
\def\FP{{\em Fortschr. Phys.} }
\def\ZP{{\em Z. Phys.} }
%


==> com_def_tex/journal_def_foster.tex <==
% A useful Journal macro
\def\Journal#1#2#3#4{{#1} {\bf #2}, #3 (#4)}

% Some useful journal names
\def\NCA{{\rm Nuovo Cimento}}
\def\NIM{{\rm Nucl. Instrum. Methods}}
\def\NIMA{{\rm Nucl. Instrum. Methods} A~}
\def\NPA{{\rm Nucl. Phys.} A~}
\def\NPB{{\rm Nucl. Phys.} B~}
\def\PLB{{\rm Phys. Lett.}  B~}
\def\PRA{{\rm Phys. Reports}  A~}
\def\PRL{{\rm Phys. Rev. Lett.} }
\def\PRD{{\rm Phys. Rev.} D~}
\def\ZPC{{\rm Z. Phys.} C~}
\def\EPC{{\rm Eur. Phys. J.} C~}
\def\CMC{{\rm Comp. Phys. Comm.} }
\def\CNPP{{\rm Comm. Nucl. Part. Phys.} }
%
\def\SJNP{{\rm Sov. J. Nucl. Phys.} }
\def\CJPB{{\rm Czech. J. Phys.} B~}
%


==> com_def_tex/newcom.tex <==
%
\newcommand{\GeVs}      {\mbox{${\rm GeV}^2$}}
\newcommand{\GeV}       {\mbox{${\rm GeV}$}}
\newcommand{\MeV}       {\mbox{${\rm MeV}$}}
\newcommand{\qsq}       {\mbox{${Q^2}$}}
\newcommand{\rhod}      {\mbox{${\rho^0}$}}
%\newcommand{\wgp}      {\mbox{${W_{\gamma p}}$}}
\newcommand{\wgp}       {\mbox{${W}$}}
\newcommand{\empz}      {\mbox{${\delta}$}}
\newcommand{\phid}      {\mbox{${\phi}$}}
\newcommand{\jpsid}     {\mbox{${J/\psi}$}}
\newcommand{\yjb}       {\mbox{${y_{_{JB}}}$}}
%
\newcommand{\ys}        {\mbox{$y_{\Sigma}$}}
\newcommand{\xes}       {\mbox{$x_{e\Sigma}$}}
\newcommand{\wes}       {\mbox{$W_{e\Sigma}$}}
\newcommand{\eda}       {\mbox{$E_{DA}^{\prime}$}}
%
\newcommand{\ra}        {\mbox{$\rightarrow$}}
\newcommand{\gsp}       {\mbox{$\gamma^* p$}}
\newcommand{\xda}       {\mbox{$x_{DA}$}}
\newcommand{\qda}       {\mbox{$Q^{2}_{DA}$}}
\newcommand{\qe}        {\mbox{$Q^{2}_{e}$}}
\newcommand{\gsubh}     {\mbox{$\gamma_{_{H}}$}}
\newcommand{\te}        {\mbox{$\theta_{e}^{\prime}$}}
\newcommand{\Ee}        {\mbox{$E_{e}^{\prime}$}}
\newcommand{\gh}        {\mbox{$\gamma_{h}$}}
\newcommand{\mrsdm}     {\mbox{MRSD$_-^{\prime}$\ }}
\newcommand{\mrsdz}     {\mbox{MRSD$_0^{\prime}$\ }}
\newcommand{\ftwo}      {\mbox{$F_{2}$}}
\newcommand{\ftwoccb}   {\mbox{$F_{2}^{c\bar c}$}}
%\newcommand{\ftwoccb}   {\mbox{$F_{2}^{c}$}}
\newcommand{\ptr}       {\mbox{$p_{T}$}}
\newcommand{\ccb}       {\mbox{$c\bar{c}$}}
\newcommand{\dspm}      {\mbox{$D^{\ast \pm}$}}
\newcommand{\ds}        {\mbox{$D^{\ast}$}}
\newcommand{\dz}        {\mbox{$D^{0}$}}
\newcommand{\mc}        {\mbox{$m_{c}$}}
\newcommand{\dm}        {\mbox{$\Delta M$}}
\newcommand{\dsp}       {\mbox{$D^{\ast +}$}}
\newcommand{\xd}        {\mbox{$x(D^{\ast})$}}
\newcommand{\ptds}      {\mbox{$p_T(D^{\ast})$}}
\newcommand{\etads}     {\mbox{$\eta(D^{\ast})$}}
\newcommand{\mkpi}      {\mbox{$M_{K\pi}$}}
\newcommand{\mdz}       {\mbox{$M(D^0)$}}
\newcommand{\mkpipis}   {\mbox{$M_{K\pi\pi_{s}}$}}
\newcommand{\ps}        {\mbox{$\pi_{s}$}}
\newcommand{\sleq} {\raisebox{-.6ex}{${\textstyle\stackrel{<}{\sim}}$}}
\newcommand{\sgeq} {\raisebox{-.6ex}{${\textstyle\stackrel{>}{\sim}}$}}
\renewcommand{\thefootnote}{\arabic{footnote}}
%


==> com_def_tex/physics_rus.tex <==
%
\newcommand{\rgevs}     {\mbox{$\,$Ĵ'$^2$}}
\newcommand{\rgev}      {\mbox{$\,$Ĵ'}}
\newcommand{\rmev}      {\mbox{$\,$δ'}}
%

